Q# as a Quantum Algorithmic Language

Q# is a standalone domain-specific programming language from Microsoft for writing and running quantum programs. Like most industrial languages, it was designed without a formal specification, which can naturally lead to ambiguity in its interpretation. We aim to provide a formal language definition for Q#, placing the language on a solid mathematical foundation and enabling further evolution of its design and type system. This paper presents $\lambda$-Q#, an idealized version of Q# that illustrates how we may view Q# as a quantum Algol (algorithmic language). We show the safety properties enforced by $\lambda$-Q#'s type system and present its equational semantics based on a fully complete algebraic theory by Staton.

==> eptcsdata.tex <==
\providecommand{\firstpage}{170}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.10}{10.4204/EPTCS.394.10}}
\pdfoutput=1

